Simple theory for scotogenic dark matter with residual matter-parity

Dark matter stability can result from a residual matter-parity symmetry surviving spontaneous breaking of an extended gauge symmetry. We propose the simplest scotogenic dark matter completion of the original SVS theory (Phys.Rev. D22 (1980) 738), in which the "dark sector" particles as well as matter-parity find a natural theoretical origin in the model. We briefly comment on its main features.

==> Makefile <==
FILENAME=Simplest3311Scoto_2020_07_20
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = Simplest3311Scoto_2020_07_20.ps 
PDFFILE = Simplest3311Scoto_2020_07_20.pdf

COPY = if test -r Simplest3311Scoto_2020_07_20.toc; then cp Simplest3311Scoto_2020_07_20.toc Simplest3311Scoto_2020_07_20.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f Simplest3311Scoto_2020_07_20.aux Simplest3311Scoto_2020_07_20.log Simplest3311Scoto_2020_07_20.dvi Simplest3311Scoto_2020_07_20.toc Simplest3311Scoto_2020_07_20.out Simplest3311Scoto_2020_07_20.blg Simplest3311Scoto_2020_07_20.mtc Simplest3311Scoto_2020_07_20.mtc1 Simplest3311Scoto_2020_07_20.rel Simplest3311Scoto_2020_07_20.vrb Simplest3311Scoto_2020_07_20.end Simplest3311Scoto_2020_07_20.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" Simplest3311Scoto_2020_07_20.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	Simplest3311Scoto_2020_07_20.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	PhysBiblio.exe tex bibliography.bib './Simplest3311Scoto_2020_07_20.tex' './tcilatex.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


